Linking Representations with Multimodal Contrastive Learning

Many applications require linking individuals, firms, or locations across datasets. Most widely used methods, especially in social science, do not employ deep learning, with record linkage commonly approached using string matching techniques. Moreover, existing methods do not exploit the inherently multimodal nature of documents. In historical record linkage applications, documents are typically noisily transcribed by optical character recognition (OCR). Linkage with just OCR'ed texts may fail due to noise, whereas linkage with just image crops may also fail because vision models lack language understanding (e.g., of abbreviations or other different ways of writing firm names). To leverage multimodal learning, this study develops CLIPPINGS (Contrastively LInking Pooled Pre-trained Embeddings). CLIPPINGS aligns symmetric vision and language bi-encoders, through contrastive language-image pre-training on document images and their corresponding OCR'ed texts. It then contrastively learns a metric space where the pooled image-text embedding for a given instance is close to embeddings in the same class (e.g., the same firm or location) and distant from embeddings of a different class. Data are linked by treating linkage as a nearest neighbor retrieval problem with the multimodal embeddings. CLIPPINGS outperforms widely used string matching methods by a wide margin in linking mid-20th century Japanese firms across financial documents. A purely self-supervised model - trained only by aligning the embeddings for the image crop of a firm name and its corresponding OCR'ed text - also outperforms popular string matching methods. Fascinatingly, a multimodally pre-trained vision-only encoder outperforms a unimodally pre-trained vision-only encoder, illustrating the power of multimodal pre-training even if only one modality is available for linking at inference time.

==> figures/dataset_newspapers.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{figures/clippings_b.png}
\caption{This figure illustrates image-caption data that came from the same underlying photo news wire source.} \label{fig:data_news}
\end{figure}


==> tables/additional_newspaper_results.tex <==
\begin{table}[ht]
    \centering
    %\resizebox{\linewidth}{!}{
    \begin{threeparttable}
       \begin{tabular}{lc}
      \toprule
       & ARI \\
\cmidrule{1-2}

\multicolumn{2}{l}
{\textbf{\textit{Panel A: Zero-shot CLIP}}} \\
Visual Linking & 	
0.182 \\
Language Linking   & 0.291 \\
Multimodal Linking  & 0.314 \\


\multicolumn{2}{l}
{\textbf{\textit{Panel B: Only Supervised Training}}} \\
Visual Linking & 	
 0.200 \\
Language Linking   & 0.303 \\
Multimodal Linking  & 	
0.559 \\     \bottomrule 
    \end{tabular}
    \end{threeparttable}
 %}
    \caption{Noisy Duplicate Ablations: This table reports the adjusted rand index for detecting noisy duplicated image-caption pairs in a historical newspaper corpus, using CLIP off-the-shelf (Panel A) and using only supervised training, with no language-image pre-training (Panel B).}
      \label{add_news_matching_results}
\end{table}


==> tables/newspaper_results.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{threeparttable}
       \begin{tabular}{lc}
      \toprule
       & ARI \\
\cmidrule{1-2}

\multicolumn{2}{l}{\textbf{\textit{Panel A: String-Matching}}} \\
Jaccard similarity & 40.3 \\ \\
\multicolumn{2}{l}{\textbf{\textit{Panel B: Language-Image Self-Supervised Training}}} \\
Visual Linking & 40.7 \\
Language Linking & 31.0 \\
Multimodal Linking & 43.0 \\ \\
\multicolumn{2}{l}{\textbf{\textit{Panel C: Supervised Training on Linked Data}}} \\
\multicolumn{2}{l}{\textbf{\textit{\ \ with Language-Image Pre-training}}} \\
Visual Linking & 59.7 \\
Language Linking   & 38.9 \\
Multimodal Linking  & \textbf{61.5} \\
      \bottomrule 
    \end{tabular}
    \end{threeparttable}
 }
    \caption{Detecting Noisy Image-Caption Duplicates: This table reports adjusted rand index on the test set using a variety of different methods for detecting noisy duplicated image-caption pairs in a historical newspaper corpus.}
      \label{news_matching_results}
\end{table}


==> tables/repro_checklist.tex <==
% \usepackage{tabularray}
\begin{longtblr}[
 caption = {Reproducibility checklist},
  label = {tab:rep_cl},
]{
  width = \linewidth,
  colspec = {Q[467]Q[106]Q[369]},
  row{1} = {c},
  cell{2}{1} = {c=3}{0.942\linewidth},
  cell{6}{1} = {c=3}{0.942\linewidth},
  cell{15}{1} = {c=3}{0.942\linewidth},
  cell{21}{1} = {c=3}{0.942\linewidth},
  hlines,
}
\textbf{Item}                                                                                                                                                                    & \textbf{Response} & \textbf{Comment}                                                                                                                                                                                                    \\
\textbf{For all models and algorithms presented, check if you include:}                                                                                                          &                   &                                                                                                                                                                                                                     \\
{A clear description of the mathematical setting,\\  algorithm, and/or model.}                                                                                                   & Yes               &                                                                                                                                                                                                                     \\
A clear explanation of any assumptions.                                                                                                                                          & Yes               &                                                                                                                                                                                                                     \\
{An analysis of the complexity\\  (time, space, sample size) of any algorithm.}                                                                                                  & NA                & {Complexity can depend upon \\ application-specific architecture\\  and methods. We are using\\ transformer-based models within our\\ framework and we have reported \\ the time profile and other related details} \\
\textbf{For any theoretical claim, check if you include:}                                                                                                                        &                   &                                                                                                                                                                                                                     \\
A clear statement of the claim.                                                                                                                                                  & Yes               &                                                                                                                                                                                                                     \\
A complete proof of the claim.                                                                                                                                                   & Yes               &                                                                                                                                                                                                                     \\
\textbf{For all datasets used, check if you include:}                                                                                                                            &                   &                                                                                                                                                                                                                     \\
{The relevant statistics, such\\  as number of examples}                                                                                                                         & Yes               &                                                                                                                                                                                                                     \\
The details of train / validation / test splits                                                                                                                                  & Yes               &                                                                                                                                                                                                                     \\
{An explanation of any data that\\  were excluded, and all pre-processing step.}                                                                                                 & Yes               &                                                                                                                                                                                                                     \\
{A link to a downloadable version \\ of the dataset or simulation environment}                                                                                                   & No                & External links are not permitted                                                                                                                                                               \\
{For new data collected, a complete\\  description of the data collection process,\\  such as instructions to annotators \\ and methods for quality control.}                    & Yes               & {This mostly involved data extraction\\ pipelines (the code has been shared) \\ and an annotation effort (outlined)}                                                                                                \\
\textbf{For all shared code related to this work, check if you include:}                                                                                                         &                   &                                                                                                                                                                                                                     \\
Specification of dependencies.                                                                                                                                                   & Yes               &                                                                                                                                                                                                                     \\
Training code.                                                                                                                                                                   & Yes               & {The code will also be made publicly \\ available after the review process}                                                                                                                                         \\
Evaluation codes                                                                                                                                                                 & Yes               &                                                                                                                                                                                                                     \\
(Pre-)trained model(s).                                                                                                                                                          & No                & {Each model's size exceeds 700 MB \\ (same as CLIP), so it can't fit\\ into the submission file. \\ They will be made publicly\\  available after the review process}                                               \\
{README file includes table of results \\ accompanied by precise \\ command to run to produce those results}                                                                     & Yes               &                                                                                                                                                                                                                     \\
\textbf{For all reported experimental results, check if you include:}                                                                                                            &                   &                                                                                                                                                                                                                     \\
{The range of hyper-parameters considered,\\  method to select the best hyper-parameter\\  configuration, and specification of all \\ hyper-parameters used to generate results} & Yes               &                                                                                                                                                                                                                     \\
The exact number of training and evaluation runs.                                                                                                                                & Yes               &                                                                                                                                                                                                                     \\
{A clear definition of the specific\\  measure or statistics used to report results.}                                                                                            & Yes               &                                                                                                                                                                                                                     \\
{A description of results with \\ central tendency (e.g. mean)  variation (e.g. error bars).}                                                                                    & NA                &                                                                                                                                                                                                                     \\
{The average runtime for each result,\\  or estimated energy cost.}                                                                                                              & Yes               & {Both training and inference times \\ have been reported}                                                                                                                                                           \\
A description of the computing infrastructure used                                                                                                                               & Yes               &                                                                                                                                                                                                                    
\end{longtblr}


